Reliable Label Correction is a Good Booster When Learning with Extremely Noisy Labels

Learning with noisy labels has aroused much research interest since data annotations, especially for large-scale datasets, may be inevitably imperfect. Recent approaches resort to a semi-supervised learning problem by dividing training samples into clean and noisy sets. This paradigm, however, is prone to significant degeneration under heavy label noise, as the number of clean samples is too small for conventional methods to behave well. In this paper, we introduce a novel framework, termed as LC-Booster, to explicitly tackle learning under extreme noise. The core idea of LC-Booster is to incorporate label correction into the sample selection, so that more purified samples, through the reliable label correction, can be utilized for training, thereby alleviating the confirmation bias. Experiments show that LC-Booster advances state-of-the-art results on several noisy-label benchmarks, including CIFAR-10, CIFAR-100, Clothing1M and WebVision. Remarkably, under the extreme 90\% noise ratio, LC-Booster achieves 92.9\% and 48.4\% accuracy on CIFAR-10 and CIFAR-100, surpassing state-of-the-art methods by a large margin.

==> sections/7.checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{The improvement of LC-Booster shrinks with less label noise.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Sec.~\ref{sec:reco}}
  \item Did you include complete proofs of all theoretical results?
    \answerYes{See the supplementary material.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please refer to the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sec.~\ref{sec:impl} and the supplementary material.}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Running multiple times is not affordable to us.}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the supplementary material.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/abl_module.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c}
        \toprule
         ReCo & H-Aug. & CIFAR-10 & CIFAR-100 \\
         \hline
         && 83.9 & 31.5 \\
         \checkmark & &85.3 & 36.3 \\
         & \checkmark &89.8 & 41.8 \\
         \checkmark &\checkmark &\textbf{92.9}&\textbf{48.4} \\
         \bottomrule
    \end{tabular}
    \caption{Evaluation of ReCo and H-Aug. in the proposed framework. The noise type is 90\% symmetric noise for both CIFAR-10 and CIFAR-100. \textbf{Bold entries} are best results.}
    \label{tab:abl_module}
\end{table}


==> tables/abl_relabel_side.tex <==
\begin{SCtable}[][t]\setlength{\tabcolsep}{5pt}
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        Epoch(s) & 50 & 100 & 150 & 200 & 250 & 100\&200 \\
        \hline
        Test Acc. (\%) & 91.9 & \textbf{92.9} & 91.5 & 90.3 & 89.7 & 92.7 \\
        \bottomrule
    \end{tabular}
    \caption{Exploring which epoch(s) to perform ReCo. The last column means re-labeling twice at the 100th and 200th epoch. The best result is marked in \textbf{bold}.}
    \label{tab:relabel}
\end{SCtable}

==> tables/abl_tau.tex <==
\begin{table}[h]
    \centering
    \footnotesize
    \begin{tabular}{c|c|c|c|c|c}
        \toprule
         $\tau_{ps}$ & 0.0 & 0.5  & 0.7 & 0.8 & 0.95 \\
         \hline
         $|\hat{\mathcal{S}}_{ps}|$ &50000   &42641  &29715 & 13405 & 483 \\
         Label Pres. (\%) & 84.6 & 91.5 & 97.4 & 99.1 & 100.0 \\
         Test Acc. (\%) & 84.9 & 90.5 & 93.4 & \textbf{92.9} & 91.3 \\
         \bottomrule
    \end{tabular}
    \caption{Exploration of different $\tau_{ps}$. $\hat{\mathcal{S}}_{ps}$ is defined in Eq.~\ref{eq:S_hat} as the set of revised samples. Label Pres. denotes the label precision of $\hat{\mathcal{S}}_{ps}$. The last row is test accuracy on CIFAR-10 with 90\% symmetric noise. The best result is marked in \textbf{bold}.}
    \label{tab:tau}
\end{table}

==> tables/clothing1m.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabular}	{l |c }
		\toprule	 	
			Method  & Test Accuracy \\
			\midrule			
			Cross-Entropy & 69.21 \\
			F-correction~\citep{patrini2017making}  &69.84\\		
			M-correction~\citep{arazo2019unsupervised}&  71.00 \\			
			Joint-Optim~\citep{tanaka2018joint}  & 72.16\\			
			Meta-Cleaner~\citep{zhang2019metacleaner} & 72.50\\
			Meta-Learning~\citep{li2019learning}  & 73.47\\				
			P-correction~\citep{yi2019probabilistic}&73.49\\
			AFM~\cite{peng2020suppressing} &74.12\\
			SMP ~\cite{han2019deep} &74.45\\
			DivideMix ~\cite{li2020dividemix} & 74.76\\
			ELR+ ~\citep{liu2020early} &74.81\\
			LongReMix ~\citep{cordeiro2021longremix} &74.38\\
			DM-AugDesc ~\citep{nishi2021augmentation} &75.11 \\
% 			PGDF ~\citep{chen2021sample} &75.19\\
			\midrule
			Ours & \textbf{75.23}\\
		\bottomrule
	\end{tabular}
	%}
	\caption{Comparison with state-of-the-art methods in test accuracy (\%) on Clothing1M. Results for baseline methods are cited from original papers. The best entry is marked in \textbf{bold}.}
	\label{tab:c1m}	
\end{table}		

==> tables/webvision.tex <==
\begin{table}[ht]
	\centering
% 	\small
	\scriptsize
	\begin{tabular}	{l |c|c|c|c }
		\toprule	 	
			\multirow{2}{*}{Method}  & \multicolumn{2}{c|}{WebVision} & \multicolumn{2}{c}{ILSVRC12}\\
			\cmidrule{2-5}
			& Top1 & Top5& Top1 & Top5\\
			\midrule			
			F-correction~\citep{patrini2017making} & 61.12 & 82.68&  57.36 &82.36\\		
			Decoupling~\citep{malach2017decoupling} & 62.54 &84.74 & 58.26 &82.26\\
			D2L~\citep{ma2018dimensionality} &62.68 &84.00&  57.80 & 81.36 \\
			MentorNet~\citep{jiang2018mentornet}  &63.00 &81.40&  57.80 &79.92 \\
			Co-teaching~\citep{han2018co} & 63.58 & 85.20 & 61.48 & 84.70\\			
			Iterative-CV~\citep{chen2019understanding} & 65.24 &85.34 & 61.60 & 84.98 \\
			DivideMix~\citep{li2020dividemix} & 77.32 & 91.64 & 75.20 & 90.84\\
			LongReMix \cite{cordeiro2021longremix} & 78.92 & \textbf{92.32} & - & - \\
            NGC \cite{wu2021ngc} & \textbf{79.16} & 91.84 & 74.44 & 91.04 \\
			\midrule
			Ours & 78.29 & 92.18 & \textbf{75.44} & \textbf{91.26} \\
		\bottomrule
	\end{tabular}
	
	\caption{Comparison with state-of-the-art methods trained on (mini) WebVision dataset. Numbers denote top-1 (top-5) accuracy (\%) on the WebVision validation set and the ILSVRC12 validation set. Results for baseline methods are cited from their original papers. \textbf{Bold entries} are best results.}
	\label{tab:webvision}
\end{table}		

